Forging Vision Foundation Models for Autonomous Driving: Challenges, Methodologies, and Opportunities

The rise of large foundation models, trained on extensive datasets, is revolutionizing the field of AI. Models such as SAM, DALL-E2, and GPT-4 showcase their adaptability by extracting intricate patterns and performing effectively across diverse tasks, thereby serving as potent building blocks for a wide range of AI applications. Autonomous driving, a vibrant front in AI applications, remains challenged by the lack of dedicated vision foundation models (VFMs). The scarcity of comprehensive training data, the need for multi-sensor integration, and the diverse task-specific architectures pose significant obstacles to the development of VFMs in this field. This paper delves into the critical challenge of forging VFMs tailored specifically for autonomous driving, while also outlining future directions. Through a systematic analysis of over 250 papers, we dissect essential techniques for VFM development, including data preparation, pre-training strategies, and downstream task adaptation. Moreover, we explore key advancements such as NeRF, diffusion models, 3D Gaussian Splatting, and world models, presenting a comprehensive roadmap for future research. To empower researchers, we have built and maintained https://github.com/zhanghm1995/Forge_VFM4AD, an open-access repository constantly updated with the latest advancements in forging VFMs for autonomous driving.

==> mind_map.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=white!100!red, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}
    {
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge={darkgray, line width=1pt},
                % s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt},
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                where level=1{text width=6em,font=\scriptsize,}{},
                where level=2{text width=7em,font=\scriptsize,}{},
                where level=3{text width=7em,font=\scriptsize,}{},
                where level=4{text width=8em,font=\scriptsize,}{},
            [~~Forging Vision Foundation Models for Autonomous Driving~~, ver, 
                [~~Data Preparation, ver,
                    [Generative Adversarial \\ Network
                        [{\textit{e.g.,} DriveGAN, DeepRoad, SurfelGAN,  LiDARGAN}, leaf, text width=30em]
                    ]
                    [Diffusion Models
                        [{\textit{e.g.,} GeoDiffusion, DriveDreamer, DrivingDiffusion}, leaf, text width=30em]
                   ]
                   [Neural Radiance Field
                        [{\textit{e.g.,} READ, MapNeRF, UniSim, MARS, S-NeRF, RoMe, StreetSurf}, leaf, text width=30em]
                   ]
                ]
                [~~~Self-supervised \\ Training Paradigms, ver
                [Contrastive-based 
                        [{\textit{e.g.,} PointContrast, DepthContrast, SegContrast, ProposalContrast },leaf, text width=30em]
                    % [Open-Vocabulary \\ Semantic Segmentation 
                    %     [{\textit{e.g.,} LSeg~\cite{li2022languagedriven}, Segment Anything~\cite{kirillov2023segment}, FastSAM~\cite{zhao2023fast}, MobileSAM~\cite{mobile_sam},\\ Track Anything Model (TAM)~\cite{yang2023track}}, leaf, text width=25em]
                    % ]
                    % [Open-Vocabulary 3D \\Scene Representation
                    %     [{\textit{e.g.,} CLIP-NERF~\cite{wang2022clip}, LERF~\cite{lerf2023}, DFF~\cite{kobayashi2022decomposing}},leaf, text width=25em]
                    % ]
                    % [Affordances
                    %     [{\textit{e.g.,} Affordance Diffusion~\cite{ye2023affordance}, VRB~\cite{bahl2023affordances}},leaf, text width=25em]
                    % ]
                ]
                [Reconstruction-based
                        [{\textit{e.g.,} VoxelMAE, GeoMAE, MaskPoint, MAELi,  BEV-MAE, IAE, Occupancy-MAE },leaf, text width=30em]
                ]
                [Rendering-based
                        [{\textit{e.g.,} Ponder, Ponderv2, PRED, UniPAD, RenderOcc, SelfOcc },leaf, text width=30em]
                ]
                [World Model
                        [{\textit{e.g.,} GAIA-1, ADriver-I, MLLM, OccWorld, MUVO,  Drive-WM },leaf, text width=30em]
                ]
                [Distillation-based
                        [{\textit{e.g.,} SLidR, ST-SLidR, SEAL },leaf, text width=30em]
                ]
                % [Other Categories
                %         [{\textit{e.g.,}  Self-supervised Scene Flow~\cite{erccelik20223d}},leaf, text width=30em]
                % ]
                ]
                [~~~~~Adapatation, ver,
                    [SAM
                    [{\textit{e.g.,} SPINO}, leaf, text width=30em]
                    ]
                    [ CLIP
                        [{\textit{e.g.,} LSeg, MaskCLIP, FC-CLIP, ODISE, CLIP2Scene, OVO, POP-3D}, leaf, text width=30em]
                   ]
                   [ LLMs \& VLMs
                        [{\textit{e.g.,} GPT-Driver, LanguageMPC, Drive Like a Human}, leaf, text width=30em]
                   ]
                ]
            ]
        \end{forest}
    }
    \caption{\textbf{Research tree of this survey.} To forge vision foundation models, we mainly recognize three key components, each with various methods. And we also exemplify several representative works for reference.}
    \label{mind_map}
\end{figure*}

%%%% ZHM: Adapted from Foundation Models in Robotics: Applications, Challenges, and the Future


==> tables/charter3.tex <==
\begin{table*}[t]
\footnotesize
\centering
\caption{Data Preparation-Summary of techniques for data generation .} 
\resizebox{\textwidth}{!}{
    \begin{tabular}{l|ccp{10cm}}
    \toprule
        \textbf{Methods} & {\textbf{Year}} & {\textbf{Category}} & {\textbf{Contributions}} \\ \hline

        Image-to-Image Translation with Conditional Adversarial Networks~\cite{isola2017image}  & 2023 &  GAN & conditional adversarial networks are promising for many image-to-image translation tasks, especially those involving highly structured graphical outputs. \\ 
        
        CycleGAN & 2023 &  GAN & capturing special characteristics of one image collection and figuring out how these characteristics could be translated into the other image collection. \\ 

        BicycleGAN & 2023 &  GAN & The proposed method encourages bijective consistency between the latent encoding and output modes. We present a systematic comparison of our method and other variants on both perceptual realism and diversity. \\

        
        Pix2PixHD & 2023 &  GAN & this paper suggest that conditional GANs are able to synthesize high-resolution photo-realistic imagery without any hand-crafted losses or pre-trained networks. \\
                
        MUNIT & 2023 &  GAN & By sampling different style codes, the model is able to produce diverse and multimodal outputs.   Moreover, the decomposition of content and style spaces allows our framework to perform example-guided image translation, in which the style of the translation outputs are controlled by a user-provided example image in the target domain. \\ 

        TGAN & 2023 &  GAN &  The generative model that can efficiently capture the latent space of the time dimension in videos. It also enables a natural extension to an application such as frame interpolation. The alternative parameter clipping method for WGAN that significantly stabilizes the training of the networks that have advanced structure. \\
        
        MCVD~\cite{NEURIPS2022_94461854} & 2022 & Diffusion & Obtain SOTA video prediction and interpolation results with randomly masked conditional video diffusion models. \\
        
        FDM~\cite{NEURIPS2022_b2fe1ee8} & 2022 & Diffusion &  Meta-learning training objective encourages model can be flexibly conditioned on any number of frames at any time in the past and future and be flexibly marginalized \\

        GeoDiffusion~\cite{chen2023geodiffusion} & 2023 & Diffusion & The generated images of layout-to-image models can be beneficial to training object detectors for the first time. \\

        DrivingDiffusion~\cite{li2023drivingdiffusion}  & 2023 & Diffusion & generates realistic multi-view driving scene videos from 3D layouts, ensuring spatial-temporal consistency and enhancing autonomous driving simulations \\
        DriveDreamer~\cite{wang2023drivedreamer}  & 2023 &  Diffusion & introduce the Autonomous-driving Diffusion Model and a two-stage training pipeline  to generate high-quality driving videos and realistic driving policies \\
        
        MagicDrive~\cite{gao2023magicdrive}   & 2023 &  Diffusion &  introduce geometric conditions encoding achieving 3D geometry controls \\
        
        READ~\cite{li2023read} & 2023 & NerF & To synthesize large scale photo-realistic scenarios on a PC. \\

        MapNeRF~\cite{wu2023mapnerf} & 2023 & NerF & 
        Incorporate commonly used map priors in AD scenes into neural radiance fields to improve the out-of-trajectory driving view synthesis. \\

        UniSim~\cite{yang2023unisim} & 2023 & NerF &  
        Improve over SoTA and generates realistic sensor data with much lower domain gap. \\
        
        MARS (ModulAr and Realistic Simulator)~\cite{wu2023mars} & 2023 &  Nerf &   build an instance-aware,  open-sourced modular framework for photo-realistic autonomous driving simulation based on NeRFs. \\

        LiDAR-NeRF~\cite{tao2023lidar} & 2023 &  Nerf & leverages NeRF to facilitate the joint learning of geometry and the attributes of 3D points.\\

        NeRF-LiDAR~\cite{zhang2023nerf}  & 2023 &  Nerf & utilizes real images and point cloud data collected by self-driving cars to learn the 3D scene representation, point cloud generation and label rendering. \\
        
        
        \bottomrule
        
    \end{tabular}
}

\label{tab:dataset_tab}
\end{table*}

==> tables/charter4_1.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=white!70!red, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}
    {
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge={darkgray, line width=1pt},
                % s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt},
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                where level=1{text width=6em,font=\scriptsize,}{},
                where level=2{text width=7em,font=\scriptsize,}{},
                where level=3{text width=7em,font=\scriptsize,}{},
                where level=4{text width=8em,font=\scriptsize,}{},
            [Self-training Paradigms for AD, ver, 
                [Representation \\ and Framework, ver,
                    [Representation \\ and Framework
                        [{e.g. Lee et al.~\cite{lee2018context}, BicycleGAN~\cite{zhu2017toward}, MUNIT~\cite{huang2018multimodal}, Augmented GAN~\cite{bowles2018gan}}, leaf, text width=25em]
                    ]
                    [Diffusion Models
                        [{e.g. GeoDiffusion~\cite{chen2023geodiffusion}, DriveDreamer~\cite{wang2023drivedreamer}, DrivingDiffusion~\cite{li2023drivingdiffusion}}, leaf, text width=30em]
                   ]
                   [Neural Radiance Field
                        [{e.g. READ~\cite{li2023read}, MapNeRF~\cite{wu2023mapnerf}, UniSim~\cite{yang2023unisim}, MARS~\cite{wu2023mars}, S-NeRF~\cite{xie2023s}, RoMe~\cite{mei2023rome}, \\ StreetSurf~\cite{guo2023streetsurf}}, leaf, text width=30em]
                   ]
                ]
                [Contrastive, ver
                    [Contrastive-based 
                            [{e.g. PointContrast~\cite{xie2020pointcontrast}, DepthContrast~\cite{zhang2021self}, SegContrast~\cite{nunes2022segcontrast}, ProposalContrast~\cite{yin2022proposalcontrast} },leaf, text width=25em]
                        % [Open-Vocabulary \\ Semantic Segmentation 
                        %     [{e.g. LSeg~\cite{li2022languagedriven}, Segment Anything~\cite{kirillov2023segment}, FastSAM~\cite{zhao2023fast}, MobileSAM~\cite{mobile_sam},\\ Track Anything Model (TAM)~\cite{yang2023track}}, leaf, text width=25em]
                        % ]
                        % [Open-Vocabulary 3D \\Scene Representation
                        %     [{e.g. CLIP-NERF~\cite{wang2022clip}, LERF~\cite{lerf2023}, DFF~\cite{kobayashi2022decomposing}},leaf, text width=25em]
                        % ]
                        % [Affordances
                        %     [{e.g. Affordance Diffusion~\cite{ye2023affordance}, VRB~\cite{bahl2023affordances}},leaf, text width=25em]
                        % ]
                    ]
                    [Reconstruction-based
                            [{e.g. GeoMIM~\cite{liu2023geomim}, PointMAE~\cite{pang2022masked}, VoxelMAE~\cite{min2022voxel}, GeoMAE~\cite{tian2023geomae}, MaskPoint~\cite{liu2022masked}, MAELi~\cite{krispel2022maeli}, \\ BEV-MAE~\cite{lin2022bev}, IAE~\cite{yan2023implicit}, Occupancy-MAE~\cite{min2023occupancy}, PiMAE~\cite{chen2023pimae} },leaf, text width=33.5em]
                    ]
                    [Volume Rendering-based
                            [{e.g. Ponder~\cite{huang2023ponder}, Ponderv2~\cite{zhu2023ponderv2}, PRED~\cite{yang2023pred}, UniPAD~\cite{yang2023unipad}, RenderOcc~\cite{pan2023renderocc}, SelfOcc~\cite{huang2023selfocc} },leaf, text width=33.5em]
                    ]
                    [World Model-based
                            [{e.g. GAIA-1~\cite{hu2023gaia}, Zhang et al.~\cite{zhang2023learning}, ADriver-I~\cite{jia2023adriveri}, MLLM~\cite{chiang2023vicuna}, OccWorld~\cite{zheng2023occworld}, MUVO~\cite{bogdoll2023muvo} },leaf, text width=33.5em]
                    ]
                    [Distillation-based
                            [{e.g. SLidR~\cite{sautier2022image}, Mahmoud et al.~\cite{mahmoud2023self}, SEAL~\cite{liu2023segment} },leaf, text width=33.5em]
                    ]
                ]
                [Reconstruction, ver,
                    [Segment Anything \\Model
                    [{e.g. CLIPort~\cite{shridhar2021cliport}, Play-LMP~\cite{lynch2019play}, PerAct~\cite{shridhar2022peract},
                        Multi-Context Imitation~\cite{lynch2021language}, \\CACTI~\cite{mandi2022cacti}, Voltron~\cite{karamcheti2023language}}, leaf, text width=25em]
                    ]
                    [ CLIP
                        [{e.g. R3M~\cite{nair2022r3m}, SayCan~\cite{Ahn2022DoAI}, Inner Monologue~\cite{huang2022inner}, VoxPoser~\cite{VoxPoser2023}, Mahmoudieh et al.~\cite{mahmoudieh2022zeroshot}, VIP~\cite{VIP2022},\\ LIV~\cite{ma2023liv}, LOREL~\cite{nair2022a}}, leaf, text width=30em]
                   ]
                   [ LLMs \& VLMs
                        [{e.g. NL2TL~\cite{chen2023nl2tl}, Chen et al.~\cite{Chen2023}}, leaf, text width=30em]
                   ]
                ]
                [Volume Rendering, ver,
                    [Segment Anything \\Model
                    [{e.g. CLIPort~\cite{shridhar2021cliport}, Play-LMP~\cite{lynch2019play}, PerAct~\cite{shridhar2022peract},
                        Multi-Context Imitation~\cite{lynch2021language}, \\CACTI~\cite{mandi2022cacti}, Voltron~\cite{karamcheti2023language}}, leaf, text width=25em]
                    ]
                    [ CLIP
                        [{e.g. R3M~\cite{nair2022r3m}, SayCan~\cite{Ahn2022DoAI}, Inner Monologue~\cite{huang2022inner}, VoxPoser~\cite{VoxPoser2023}, Mahmoudieh et al.~\cite{mahmoudieh2022zeroshot}, VIP~\cite{VIP2022},\\ LIV~\cite{ma2023liv}, LOREL~\cite{nair2022a}}, leaf, text width=30em]
                   ]
                   [ LLMs \& VLMs
                        [{e.g. NL2TL~\cite{chen2023nl2tl}, Chen et al.~\cite{Chen2023}}, leaf, text width=30em]
                   ]
                ]
                [World Model, ver,
                    [Segment Anything \\Model
                    [{e.g. CLIPort~\cite{shridhar2021cliport}, Play-LMP~\cite{lynch2019play}, PerAct~\cite{shridhar2022peract},
                        Multi-Context Imitation~\cite{lynch2021language}, \\CACTI~\cite{mandi2022cacti}, Voltron~\cite{karamcheti2023language}}, leaf, text width=25em]
                    ]
                    [ CLIP
                        [{e.g. R3M~\cite{nair2022r3m}, SayCan~\cite{Ahn2022DoAI}, Inner Monologue~\cite{huang2022inner}, VoxPoser~\cite{VoxPoser2023}, Mahmoudieh et al.~\cite{mahmoudieh2022zeroshot}, VIP~\cite{VIP2022},\\ LIV~\cite{ma2023liv}, LOREL~\cite{nair2022a}}, leaf, text width=30em]
                   ]
                   [ LLMs \& VLMs
                        [{e.g. NL2TL~\cite{chen2023nl2tl}, Chen et al.~\cite{Chen2023}}, leaf, text width=30em]
                   ]
                ]
                [Distillation, ver,
                    [Segment Anything \\Model
                    [{e.g. CLIPort~\cite{shridhar2021cliport}, Play-LMP~\cite{lynch2019play}, PerAct~\cite{shridhar2022peract},
                        Multi-Context Imitation~\cite{lynch2021language}, \\CACTI~\cite{mandi2022cacti}, Voltron~\cite{karamcheti2023language}}, leaf, text width=25em]
                    ]
                    [ CLIP
                        [{e.g. R3M~\cite{nair2022r3m}, SayCan~\cite{Ahn2022DoAI}, Inner Monologue~\cite{huang2022inner}, VoxPoser~\cite{VoxPoser2023}, Mahmoudieh et al.~\cite{mahmoudieh2022zeroshot}, VIP~\cite{VIP2022},\\ LIV~\cite{ma2023liv}, LOREL~\cite{nair2022a}}, leaf, text width=30em]
                   ]
                   [ LLMs \& VLMs
                        [{e.g. NL2TL~\cite{chen2023nl2tl}, Chen et al.~\cite{Chen2023}}, leaf, text width=30em]
                   ]
                ]
            ]
        \end{forest}
    }
    \caption{Research Tree of forgiving vision foundation models for autonomous driving.}
    \label{mind_map}
\end{figure*}

%%%% ZHM: Adapted from Foundation Models in Robotics: Applications, Challenges, and the Future


==> tables/charter4_2.tex <==
\begin{table*}[t]
\footnotesize
\centering
\caption{Summary of techniques for data generation.} 
\resizebox{\textwidth}{!}{
    \begin{tabular}{l|ccp{10cm}p{10cm}}
    \toprule
        \textbf{Methods} & {\textbf{Year}} &{\textbf{Category}} &{\textbf{Contributions}} \\ \hline
        PointContrast~\cite{xie2020pointcontrast} & 2020 & Contrastive & Obtain SOTA video prediction and interpolation results with randomly masked conditional video diffusion models. \\
        
        GCC-3D~\cite{liang2021exploring} & 2021 & Contrastive & Meta-learning training objective that encourages model can be flexibly conditioned on any number of frames at any time in the past and future and be flexibly marginalized \\

        SegContrast~\cite{nunes2022segcontrast} & 2022 & Contrastive & The generated images of layout-to-image models can be beneficial to training object detectors for the first time. \\

        GeoMAE~\cite{tian2023geomae} & 2023 & Reconstruction & To synthesize large scale photo-realistic scenarios on a PC. \\

        PointMAE~\cite{pang2022masked} & 2022 & Reconstruction & 
        Incorporate commonly used map priors in AD scenes into neural radiance fields to improve the out-of-trajectory driving view synthesis. \\

        PiMAE~\cite{chen2023pimae} & 2023 & Reconstruction &  
        Improve over SoTA and generates realistic sensor data with much lower domain gap \\

        Ponder~\cite{huang2023ponder} & 2023 & Volume Rendering &  
        Improve over SoTA and generates realistic sensor data with much lower domain gap \\

        UniPAD~\cite{yang2023unipad} & 2023 & Volume Rendering &  
        Improve over SoTA and generates realistic sensor data with much lower domain gap \\

        RenderOcc~\cite{pan2023renderocc} & 2023 & Volume Rendering &  
        Improve over SoTA and generates realistic sensor data with much lower domain gap \\

        GAIA-1~\cite{hu2023gaia} & 2023 & Volume Rendering &  
        Improve over SoTA and generates realistic sensor data with much lower domain gap \\

        RenderOcc~\cite{pan2023renderocc} & 2023 & Volume Rendering &  
        Improve over SoTA and generates realistic sensor data with much lower domain gap \\

        RenderOcc~\cite{pan2023renderocc} & 2023 & Volume Rendering &  
        Improve over SoTA and generates realistic sensor data with much lower domain gap \\

        RenderOcc~\cite{pan2023renderocc} & 2023 & Volume Rendering &  
        Improve over SoTA and generates realistic sensor data with much lower domain gap \\

        RenderOcc~\cite{pan2023renderocc} & 2023 & Volume Rendering &  
        Improve over SoTA and generates realistic sensor data with much lower domain gap \\
        
        \bottomrule
        
    \end{tabular}
}

\label{tab:dataset_tab}
\end{table*}
